Detecting Check-Worthy Claims in Political Debates, Speeches, and Interviews Using Audio Data

Developing tools to automatically detect check-worthy claims in political debates and speeches can greatly help moderators of debates, journalists, and fact-checkers. While previous work on this problem has focused exclusively on the text modality, here we explore the utility of the audio modality as an additional input. We create a new multimodal dataset (text and audio in English) containing 48 hours of speech from past political debates in the USA. We then experimentally demonstrate that, in the case of multiple speakers, adding the audio modality yields sizable improvements over using the text modality alone; moreover, an audio-only model could outperform a text-only one for a single speaker. With the aim to enable future research, we make all our data and code publicly available at https://github.com/petar-iv/audio-checkworthiness-detection.

==> tables/all_results.tex <==
% \begin{table*}[th]
%   \caption{Best results with textual models over the full multimodal dataset (multiple speakers)}
%   \label{tab:results-multiple-speakers-textual}
%   \centering
%   % \resizebox{\textwidth}{!}{%
%   \small
%   % \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Model} & \textbf{\makecell{Train dataset \\variant}} & \textbf{MAP(test)} \\
%     \midrule
%     1 & BERT & 1:1 & 37.15 \\
%     \hline
%     2 & \makecell{SVM with \\TF.IDF} & x15 & 23.92 \\
%     \hline
%     3 & \makecell{Feedforward network with\\named entities count} & x15 & 22.28 \\
%     \bottomrule
%   \end{tabular}
%   % }
% \end{table*}

% \begin{table*}[th]
%   \caption{Best results with audio models over the full multimodal dataset (multiple speakers)}
%   \label{tab:results-multiple-speakers-audio}
%   \centering
%   % \resizebox{\textwidth}{!}{%
%   % \small
%   % \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Model} & \textbf{\makecell{Train dataset \\variant}} & \textbf{\makecell{Audio segments\\variant}} & \textbf{MAP(test)} \\
%     \midrule
%     1 & HuBERT & x30 & Original & 25.26 \\
%     \hline
%     2 & wav2vec 2.0 & x15 & Original & 23.65 \\
%     \hline
%     3 & data2vec-audio & x30 & Reduced noise & 23.30 \\
%     \bottomrule
%   \end{tabular}
%   % }
% \end{table*}

% \begin{table*}[t]
%   \caption{Best results with audio models utilizing knowledge alignment over the full multimodal dataset (multiple speakers)}
%   \label{tab:results-multiple-speakers-aligned-audio}
%   \centering
%   % \resizebox{\textwidth}{!}{%
%   % \small
%   % \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Model} & \textbf{\makecell{Train dataset \\variant}} & \textbf{\makecell{Audio segments\\variant}} & \textbf{MAP(test)} \\
%     \midrule
%     1 & data2vec-audio & \makecell{Without\\changes} & Original & 29.99 \\
%     \hline
%     2 & wav2vec 2.0 & \makecell{Without\\changes} & Original & 29.96 \\
%     \hline
%     3 & HuBERT & \makecell{Without\\changes} & Original & 27.87 \\
%     \bottomrule
%   \end{tabular}
%   % }
% \end{table*}

% \begin{table*}[t]
%   \caption{Best results with text-audio ensembles over the full multimodal dataset (multiple speakers)}
%   \label{tab:results-multiple-speakers-ensembles}
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \small
%   \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Ensemble type} & \textbf{Model} & \textbf{\makecell{Train dataset \\variant}} & \textbf{\makecell{Audio segments\\variant}} & \textbf{MAP(test)}  \\
%     \midrule
%     1 & \makecell{Early\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& HuBERT (Table~\ref{tab:results-multiple-speakers-audio}, row 1)} & \makecell{Without\\changes} & Original & 38.17 \\
%     \hline
%     2 & \makecell{Late\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& HuBERT (Table~\ref{tab:results-multiple-speakers-audio}, row 1)} & x15 & Original & 37.58 \\
%     \hline
%     3 & \makecell{Early\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& aligned data2vec (Table~\ref{tab:results-multiple-speakers-aligned-audio}, row 1)} & \makecell{Without\\changes} & Original & 37.35 \\
%     \hline
%     4 & \makecell{Late\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& aligned data2vec (Table~\ref{tab:results-multiple-speakers-aligned-audio}, row 1)} & x30 & Original & 37.24 \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table*}

% \begin{table}[h]
%   \caption{Best results with text-audio ensembles over the full multimodal dataset (multiple speakers)}
%   \label{tab:results-multiple-speakers-ensembles}
%   \centering
%   \resizebox{\textwidth}{!}{%
%   \small
%   \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c c c}
%     \toprule
%     \textbf{Row} & \textbf{\makecell{Ensemble\\type}} & \textbf{Model} & \textbf{\makecell{Train\\dataset}} & \textbf{\makecell{Audio\\segments}} & \textbf{MAP(test)}  \\
%     \midrule
%     1 & \makecell{Early\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& HuBERT (Table~\ref{tab:results-multiple-speakers-audio}, row 1)} & \makecell{Without\\changes} & Original & 38.17 \\
%     \hline
%     2 & \makecell{Late\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& HuBERT (Table~\ref{tab:results-multiple-speakers-audio}, row 1)} & x15 & Original & 37.58 \\
%     \hline
%     3 & \makecell{Early\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& aligned data2vec (Table~\ref{tab:results-multiple-speakers-aligned-audio}, row 1)} & \makecell{Without\\changes} & Original & 37.35 \\
%     \hline
%     4 & \makecell{Late\\fusion} & \makecell{BERT (Table~\ref{tab:results-multiple-speakers-textual}, row 1) \\ \& aligned data2vec (Table~\ref{tab:results-multiple-speakers-aligned-audio}, row 1)} & x30 & Original & 37.24 \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}


==> tables/single_speaker.tex <==
% \begin{table*}[t]
%   \caption{Best results with textual models over the single speaker (Trump) subset of the multimodal dataset}
%   \label{tab:results-single-speaker-textual}
%   \centering
%   \small
%   % \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Model} & \textbf{MAP(test)} \\
%     \midrule
%     1 & BERT & 32.67 \\
%     \hline
%     2 & \makecell{SVM with \\TF.IDF} & 26.93 \\
%     \hline
%     3 & \makecell{Feedforward network with\\named entities count} & 21.93 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{table*}[t]
%   \caption{Best results with audio models over the single speaker (Trump) subset of the multimodal dataset}
%   \label{tab:results-single-speaker-audio}
%   \centering
%   % \setlength{\tabcolsep}{3pt}
%   \begin{tabular}{l c c c}
%     \toprule
%     \textbf{Row \#} & \textbf{Model} & \textbf{\makecell{Audio segments\\variant}} & \textbf{MAP(test)} \\
%     \midrule
%     1 & wav2vec 2.0 & Reduced noise & 34.27 \\
%     \hline
%     2 & HuBERT & Original & 24.78 \\
%     \hline
%     3 & data2vec-audio & Reduced noise & 21.29 \\
%     \bottomrule
%   \end{tabular}
% \end{table*}

